Who Finishes the Job? A Study of Follow-Up Fixes and Commit Authorship on AI Coding Agent Pull Requests

AI coding agents now author a large share of pull requests (PRs) merged into popular open-source projects. A merged agent PR is usually considered finished work; yet, prior studies have reported issues in agent code after the merge (e.g., code smells and static-analysis issues). However, little is known about how often a merged agent PR is fixed afterward, and who actually authors the fixing. In this paper, we follow 6,774 merged agent PRs across five AI coding agents (OpenAI Codex, GitHub Copilot, Devin, Cursor, and Claude Code) from the AIDev-pop dataset (open-source repositories with at least 500 stars) into their follow-up fixes, against a baseline of 5,044 contemporaneous human PRs from the same repositories. We link each merge to its candidate fixes, verify every candidate with human annotators and an LLM judge that matches human-level agreement (binary Cohen's Kappa=0.78 against a human-human K=0.77, Direct-fix precision 90%), and attribute the fixing work at the PR and the commit level. Our findings show that (1) merged agent PRs attract verified fixes at 1.62 times the odds of merged human PRs in the same repositories over the same period of time; (2) 69.6% of verified fixes in agent merges come from the same agent; and (3) 76.4% of the verified fix PRs are agent-authored throughout all commits. These results show that agents currently largely finish their own job, but their merges still require fixing more often than human merges.

==> sections/tables/table_related-work.tex <==
\begin{table*}[t]
  \centering
  \footnotesize
  \caption{Empirical measurement studies of agentic pull requests.
           \emph{Dataset (N)} is the agent-side cohort; \emph{Human PRs} is
           the human comparison cohort, if any (\checkmark{} $=$ human
           comparison without a population-matched count); counts are PRs
           except for \citet{sawada2026maintenance}, which matches at file
           level.}
  \label{tab:related-work}
  \setlength{\tabcolsep}{5pt}
  \begin{tabular}{@{}p{0.17\linewidth}p{0.17\linewidth}c c p{0.40\linewidth}@{}}
    \toprule
    \textbf{Reference} & \textbf{Dataset (N)} & \textbf{Agents} &
      \shortstack{\textbf{Human}\\\textbf{PRs}} & \textbf{Key finding} \\
    \midrule
    \citet{li2025aiteammates_se3}    & \aidev{}, 933\,k PR        & 5 & \checkmark & \aidev{} dataset; three application analyses (productivity, review dynamics, case study); agent review often bot-mediated \\
    \citet{watanabe2026agentic}      & \aidev{}, 567 PR (Claude)  & 1 & --- & 45.1\,\% of merged Claude Code PRs get $\geq$1 revision before merge \\
    \citet{duma2026reviews}          & \aidev{}, 33.6\,k PR       & 5 & --- & 61.4\,\% of agent PRs get no recorded human review \\
    \citet{ogenrwot2026modify}       & \aidev{}, 24.0\,k PR       & 5 & 5.1\,k & Agent PRs smaller, more localised than human ($\delta{=}0.54$ commits) \\
    \citet{liu2026debt}              & GH Archive, 303\,k commits & 5 & --- & 22.7\,\% of AI-introduced static issues survive to repository HEAD \\
    \citet{rahman2026survive}        & \aidev{}, 3.0\,k PR        & 5 & 2.2\,k & Agent-authored code is modified \emph{less} often post-merge (line-level HR $0.84$); its modifications skew corrective \\
    \citet{kumar2025intuition}       & 1 org, 5-mo window         & 1 & --- & Generation cost grows to dominate review cost 10.5:1 (one org) \\
    \citet{huang2026reuse}           & \aidev{} crewAI, 617 PR    & 5 & \checkmark & AI agents produce 1.87$\times$ more semantic redundancy than humans (crewAI case study) \\
    \citet{watanabe2026communicate}  & \aidev{}, 33.6\,k PR       & 5 & --- & PR-description style differs by agent, links to reviewer engagement \\
    \citet{ogenrwot2026agenticflict} & AIware corpus, 142\,k PR   & 5 & --- & 29\,k+ agent PRs carry merge conflicts (parallel dataset) \\
    \citet{chung2026lifecycles}      & \aidev{}, 29.6\,k PR       & 5 & --- & Lifecycle roles: collaborator tools are agent-initiated, assistants human-initiated; merges stay human-approved \\
    \citet{minh2026revieweffort}     & \aidev{}, 33.7\,k PR       & 4 & --- & Review-effort volume predictable from size-driven creation-time features \\
    \citet{khemissi2026referenced}   & \aidev{}, 33.6\,k PR       & 5 & --- & 4.2\,\% of agent PRs are explicitly referenced later; 95.6\,\% of references human-initiated \\
    \citet{oukhay2026reverts}        & \aidev{}, 33.6\,k PR       & 5 & 6.6\,k & 2.7\,\% of agentic PRs contain an in-PR revert (human baseline 4.7\,\%) \\
    \citet{cynthia2026postmerge}     & \aidev{}, 1.2\,k fix PR    & 5 & --- & SonarQube issues in merged Python bug-fix PRs; per-agent differences vanish per KLOC \\
    \citet{sawada2026maintenance}    & \aidev{}, 508+508 files    & 4 & 508 files & Humans author 83.2\,\% of later commits to agent-created files; only 11.7\,\% of those commits are fix-typed; agent share 2.4$\times$ higher on agent files than human files \\
    \midrule
    \textbf{This paper}              & \aidev{}-pop, 6.8\,k PR    & 5 & 5.0\,k & Agent merges candidate fixes at 1.41$\times$ and verified fixes at 1.62$\times$ the human odds within the same repositories; 69.6\,\% of the verified fixes on agent merges come from the same agent; the commits on a merged agent PR are, on average, 78.6\,\% agent-authored per PR (verified fix PRs excluded) across the four agents that sign their commits; the merges that get fixed look like those that do not at merge time \\
    \bottomrule
  \end{tabular}
\end{table*}
